Exact entanglement growth of a one-dimensional hard-core quantum gas during a free expansion

We consider the non-equilibrium dynamics of the entanglement entropy of a one-dimensional quantum gas of hard-core particles, initially confined in a box potential at zero temperature. At $t=0$ the right edge of the box is suddenly released and the system is let free to expand. During this expansion, the initially correlated region propagates with a non-homogeneous profile, leading to the growth of entanglement entropy. This setting is investigated in the hydrodynamic regime, with tools stemming from semi-classical Wigner function approach and with recent developments of quantum fluctuating hydrodynamics. Within this framework, the entanglement entropy can be associated to a correlation function of chiral twist-fields of the conformal field theory that lives along the Fermi contour and it can be exactly determined. Our predictions for the entanglement evolution are found in agreement with and generalize previous results in literature based on numerical calculations and heuristic arguments.

==> bibliography.tex <==
\begin{thebibliography}{100}

\bibitem{Odor2004} G. \'Odor,
Universality classes in nonequilibrium lattice systems,
\href{https://journals.aps.org/rmp/abstract/10.1103/RevModPhys.76.663}{Rev. Mod. Phys. {\bf76}, 663 (2004)}

\bibitem{Dziarmaga2010} J. Dziarmaga,
Dynamics of a quantum phase transition and relaxation to a steady state,
\href{https://doi.org/10.1080/00018732.2010.514702}{Adv. Phys. {\bf59}, 1063 (2010)}.

\bibitem{pem-16} P. Calabrese, F. H. L. Essler, and G. Mussardo, Quantum Integrability in Out of Equilibrium Systems,
\href{http://iopscience.iop.org/article/10.1088/1742-5468/2016/06/064001}{J. Stat. Mech. (2016) 064001}.

\bibitem{Polkovnikov2011} A. Polkovnikov, K. Sengupta, A. Silva and M. Vengalattore,
Colloquium: Nonequilibrium dynamics of closed interacting quantum systems,
\href{https://journals.aps.org/rmp/abstract/10.1103/RevModPhys.83.863}{Rev. Mod. Phys. {\bf83}, 863 (2011)}

\bibitem{Bertini2021} B. Bertini, F. Heidrich-Meisner, C. Karrasch, T. Prosen, R. Steinigeweg and M. Znidaric,
Finite-temperature transport in one-dimensional quantum lattice models,
\href{https://journals.aps.org/rmp/abstract/10.1103/RevModPhys.93.025003}{Rev. Mod. Phys. {\bf93}, 025003 (2021)}.

\bibitem{Rigol2007} M. Rigol, V. Dunjko, V. Yurovsky, and M. Olshanii,
 Relaxation in a completely integrable many-body Quantum system: An Ab initio study of the dynamics of the highly excited states of 1D lattice hard-core bosons,
\href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.98.050405}{Phys. Rev. Lett. {\bf98}, 050405 (2007)}

\bibitem{Rigol2008} M. Rigol, V. Dunjko, and M. Olshanii,
Thermalization and its mechanism for generic isolated quantum systems, 
\href{https://www.nature.com/articles/nature06838}{Nature {\bf 452}, 854 (2008)}

\bibitem{vr-16} L.~Vidmar and M.~Rigol, 
Generalized Gibbs ensemble in integrable lattice models, 
\href{http://dx.doi.org/10.1088/1742-5468/2016/06/064007}{J. Stat. Mech. (2016) 064007}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{Bertini2016} B. Bertini, M. Collura, J. De Nardis and M. Fagotti,
 Transport in out-of-equilibrium XXZ chains: Exact profiles of charges and currents, 
\href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.117.207201}{Phys. Rev. Lett. {\bf117}, 207201(2016)}.

\bibitem{Castro-Alvaredo2016} O. A. Castro-Alvaredo, B. Doyon and T. Yoshimura,
Emergent hydrodynamics in integrable quantum systems out of equilibrium,
\href{https://journals.aps.org/prx/abstract/10.1103/PhysRevX.6.041065}{Phys. Rev. X {\bf6}, 041065 (2016)}

\bibitem{Piroli2017} L. Piroli, J. De Nardis, M. Collura, B. Bertini and M. Fagotti,
 Transport in out-of-equilibrium XXZ chains: Nonballistic behavior and correlation functions,
\href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.96.115124}{Phys. Rev. B {\bf 96}, 115124 (2017)}

\bibitem{Bulchandani2017} V. B. Bulchandani, R. Vasseur, C. Karrasch and J. E. Moore,
 Solvable Hydrodynamics of Quantum Integrable Systems, 
\href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.119.220604}{Phys. Rev. Lett. {\bf 119}, 220604 (2017)}

\bibitem{DeLuca2017} M. Collura, A. De Luca and J. Viti,
 Analytic solution of the domain-wall nonequilibrium stationary states, 
\href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.97.081111}{Phys. Rev. B {\bf 97}, 081111(R) (2017)}

\bibitem{Doyon2017} B. Doyon, J. Dubail, R. Konik and T. Yoshimura,
 Large-Scale Description of Interacting One-Dimensional Bose Gases: Generalized Hydrodynamics Supersedes Conventional Hydrodynamics,
\href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.119.195301}{Phys. Rev. Lett. {\bf119}, 195301 (2017)}

\bibitem{DeLuca2017b} A. De Luca, M. Collura and J. De Nardis,
 Nonequilibrium spin transport in integrable spin chains: Persistent currents and emergence of magnetic domains, 
\href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.96.020403}{Phys. Rev. B {\bf 96}, 020403 (2017)}

\bibitem{Bulchandani2018} V. B. Bulchandani, R. Vasseur, C. Karrasch, and J. E. Moore,
 Bethe-Boltzmann hydrodynamics and spin transport in the XXZ chain, 
\href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.97.045407}{Phys. Rev. B {\bf97}, 045407 (2018)}

\bibitem{Doyon2018} B. Doyon, T. Yoshimura, and J. S. Caux,
 Soliton Gases and Generalized Hydrodynamics,
\href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.120.045301}{Phys. Rev. Lett. {\bf120}, 045301 (2018)}

\bibitem{Bastianello2019} A. Bastianello, V. Alba, and J. S. Caux
Generalized Hydrodynamics with Space- Time Inhomogeneous Interactions, 
\href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.123.130602}{Phys. Rev. Lett. {\bf123}, 130602 (2019)}

\bibitem{Mestyan2019} M. Mestyán, B. Bertini, L. Piroli and P. Calabrese,
Spin-charge separation effects in the low-temperature transport of one-dimensional Fermi gases,
\href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.99.014305}{Phys. Rev. B {\bf99}, 014305 (2019)}

\bibitem{Schemmer2019} M. Schemmer, I. Bouchoule, B. Doyon, and J. Dubail,
 Generalized Hydrodynamics on an Atom Chip,
\href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.122.090601}{Phys. Rev. Lett.{\bf 122}, 090601 (2019)}

\bibitem{Bastianello2020a} A. Bastianello, J. De Nardis, and A. De Luca,
 Generalized hydrodynamics with dephasing noise,
\href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.102.161110}{Phys. Rev. B {\bf102}, 161110 (2020)}

\bibitem{Ruggiero2020} P. Ruggiero, P. Calabrese, B. Doyon and J. Dubail,
 Quantum Generalized Hydrodynamics,
\href{https://link.aps.org/doi/10.1103/PhysRevLett.124.140603}{Phys. Rev. Lett. {\bf124}, 140603 (2020)}

\bibitem{Malvania2020} N. Malvania, Y. Zhang, Y. Le, J. Dubail, M. Rigol, and D. S. Weiss,
Generalized hydrodynamics in strongly interacting 1D Bose gases,
 \href{https://arxiv.org/abs/2009.06651}{preprint - arXiv:2009.06651 (2020)}

\bibitem{Bouchoule2020a} I. Bouchoule and J. Dubail,
 Breakdown of Tan’s relation in lossy one-dimensional Bose gases,
\href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.126.160603}{Phys. Rev. Lett. {\bf126}, 160603 (2021)}

\bibitem{Perfetto2020} G. Perfetto and B. Doyon,
Euler-scale dynamical fluctuations in non-equilibrium interacting integrable systems, 
\href{https://arxiv.org/abs/2012.06496}{preprint - arXiv:2012.06496}

\bibitem{Moller2020} F. S. M{\o}ller, G. Perfetto, B. Doyon and J. Schmiedmayer,
Euler-scale dynamical correlations in integrable systems with fluid motion, 
\href{https://scipost.org/SciPostPhysCore.3.2.016}{SciPost Phys. Core {\bf3}, 16 (2020)}

\bibitem{d-ls} B. Doyon, {\it Lecture notes on Generalised Hydrodynamics}, Les Houches Lecture notes,
\href{https://doi.org/10.21468/SciPostPhysLectNotes.18}{SciPost Phys. Lect. Notes {\bf 18} (2020)}.

\bibitem{Ilievski2017} E. Ilievski and J. De Nardis,
 Microscopic Origin of Ideal Conductivity in Integrable Quantum Models, 
\href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.119.020602}{Phys. Rev. Lett. {\bf119}, 020602 (2017)}

\bibitem{Alba2021} V. Alba, B. Bertini, M. Fagotti, L. Piroli and P. Ruggiero,
Generalized-Hydrodynamic approach to Inhomogeneous Quenches: Correlations, Entanglement and Quantum Effects,
\href{http://arxiv.org/abs/2104.00656}{preprint - arXiv:2104.00656 (2021)}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{sc-08} S. Sotiriadis and J. Cardy, 
{Inhomogeneous Quantum Quenches},
\href{http://dx.doi.org/10.1088/1742-5468/2008/11/P11003}{J. Stat. Mech. (2008) P11003}

\bibitem{Dubail2017} J. Dubail, J.-M. St\'ephan, J. Viti and P. Calabrese,
 Conformal field theory for inhomogeneous one-dimensional quantum systems: the example of non-interacting Fermi gases,
\href{https://scipost.org/SciPostPhys.2.1.002}{SciPost Phys. {\bf2}, 2 (2017)}

\bibitem{Brun2017} Y. Brun and J. Dubail,
 One-particle density matrix of trapped one-dimensional impenetrable bosons from conformal invariance,
\href{https://scipost.org/SciPostPhys.2.2.012/pdf}{SciPost Phys. {\bf2}, 012 (2017)}

\bibitem{Brun2018} Y. Brun and J. Dubail,
 The Inhomogeneous Gaussian Free Field, with application to ground state correlations of trapped 1d Bose gases, 
\href{https://www.scipost.org/SciPostPhys.4.6.037/pdf}{SciPost Phys. {\bf4}, 037 (2018)}

\bibitem{Langmann2019} E. Langmann and P. Moosavi,
Diffusive Heat Waves in Random Conformal Field Theory,
\href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.122.020201}{Phys. Rev. Lett. {\bf122}, 020201 (2019)}

\bibitem{Moosavi2019} P. Moosavi,
Inhomogeneous conformal field theory out of equilibrium,
\href{https://arxiv.org/abs/1912.04821}{preprint - arXiv:1912.04821 (2019)}

\bibitem{Ruggiero2019} P. Ruggiero, Y. Brun, and J. Dubail,
 Conformal field theory on top of a breathing one-dimensional gas of hard core bosons,
\href{https://www.scipost.org/SciPostPhys.6.4.051/pdf}{SciPost Phys. {\bf 6}, 051 (2019)}

\bibitem{Scopa2020} S. Scopa, L. Piroli and P. Calabrese,
 One-particle density matrix of a trapped Lieb Liniger anyonic gas, 
\href{https://iopscience.iop.org/article/10.1088/1742-5468/abaed1}{J. Stat. Mech. (2020) 093103}

\bibitem{Collura2020} M. Collura, A. De Luca, P. Calabrese, and J. Dubail,
 Domain wall melting in the spin-1/2 XXZ spin chain: Emergent Luttinger liquid with a fractal quasiparticle charge,
\href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.102.180409}{Phys. Rev. B {\bf 102}, 180409 (2020)}

\bibitem{Gluza2020} M. Gluza, P. Moosavi and S. Sotiriadis,
Breaking of Huygens-Fresnel principle in inhomogeneous Tomonaga-Luttinger liquids,
\href{https://arxiv.org/abs/2104.07751}{preprint - arXiv:2104.07751 (2021)}

\bibitem{Dean2019} D. S. Dean, P. Le Doussal, S. N. Majumdar, and G. Schehr,
 Noninteracting fermions in a trap and random matrix theory, 
\href{https://iopscience.iop.org/article/10.1088/1751-8121/ab098d}{J. Phys. A {\bf 52}, 144006 (2019)}

\bibitem{Dean2018} D. S. Dean, P. Le Doussal, S. N. Majumdar and G. Schehr,
 Wigner function of noninteracting trapped fermions, 
\href{https://journals.aps.org/pra/abstract/10.1103/PhysRevA.97.063614}{Phys. Rev. A {\bf97}, 063614 (2018)}

\bibitem{Smith2020} N. R. Smith, P. Le Doussal, S. N. Majumdar and G. Schehr,
Counting statistics for noninteracting fermions in a d-dimensional potential,
\href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.103.L030105}{Phys. Rev. E {\bf103}, L030105 (2021)}

\bibitem{Gautie2021} T. Gauti\'e, J.-P. Bouchaud and P. Le Doussal,
. Matrix kesten recursion, inverse-wishart ensemble and fermions in a morse potential, 
\href{https://arxiv.org/abs/2101.08082}{preprint - arXiv:2101.08082 (2021)}

\bibitem{DeBruyne2021} B. De Bruyne, D. S. Dean, P. Le Doussal, S. N. Majumdar and G. Schehr,
. Wigner function for noninteracting fermions in hard wall potentials, 
\href{https://arxiv.org/abs/2104.05068}{preprint - arXiv:2104.05068 (2021)}

\bibitem{Calabrese2006} P. Calabrese and J. Cardy,
 Time dependence of correlation functions following a quantum quench,
\href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.96.136801}{Phys. Rev. Lett. {\bf 96}, 136801 (2006)}

\bibitem{Calabrese2007a} P. Calabrese and J. Cardy,
 Quantum quenches in extended systems, 
\href{https://iopscience.iop.org/article/10.1088/1742-5468/2007/06/P06008}{J. Stat. Mech. (2007) P06008}

\bibitem{Caux2013} J. S. Caux and F. H.L. Essler,
 Time evolution of local observables after quenching to an integrable model, 
\href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.110.257203}{Phys. Rev. Lett. {\bf110}, 257203 (2013)}

\bibitem{Brockmann2014} M. Brockmann, B. Wouters, D. Fioretto, J. De Nardis, R. Vlijm and J. S. Caux,
Quench action approach for releasing the Néel state into the spin-1/2 XXZ chain, 
\href{https://iopscience.iop.org/article/10.1088/1742-5468/2014/12/P12009}{J. Stat. Mech. (2014)  P12009}

\bibitem{Ilievski2015} E. Ilievski, J. De Nardis, B. Wouters, J. S. Caux, F. H.L. Essler and T. Prosen,
 Complete Generalized Gibbs Ensembles in an Interacting Theory, 
\href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.115.157201}{Phys. Rev. Lett. {\bf115}, 157201 (2015)}

\bibitem{Caux2016} J. S. Caux,
 The Quench Action, 
\href{https://iopscience.iop.org/article/10.1088/1742-5468/2016/06/064006}{J. Stat. Mech. (2016) 064006}

\bibitem{Calabrese2005} P. Calabrese and J. Cardy,
 Evolution of entanglement entropy in one-dimensional systems,
\href{https://iopscience.iop.org/article/10.1088/1742-5468/2005/04/P04010}{J. Stat. Mech. (2005) 04010}

\bibitem{Alba2017} V. Alba and P. Calabrese,
 Entanglement and thermodynamics after a quantum quench in integrable systems, 
\href{https://www.pnas.org/content/114/30/7947https://www.pnas.org/content/114/30/7947.abstract}{PNAS {\bf114}, 7947 (2017)}

\bibitem{ac-18} V. Alba and P. Calabrese, Entanglement dynamics after quantum quenches in generic integrable systems, 
\href{https://scipost.org/10.21468/SciPostPhys.4.3.017}{SciPost Phys. {\bf 4}, 017 (2018)}.

\bibitem{c-20} P. Calabrese, {\it Entanglement spreading in non-equilibrium integrable systems}, 
Lectures for Les Houches Summer School on ``Integrability in Atomic and Condensed Matter Physics", 
\href{https://doi.org/10.21468/SciPostPhysLectNotes.20}{SciPost Phys. Lect. Notes 20 (2020)}.

\bibitem{bfpc-18} B.~Bertini, M.~Fagotti, L.~Piroli, and P.~Calabrese, {Entanglement evolution and generalised hydrodynamics: noninteracting systems}, 
\href{https://doi.org/10.1088/1751-8121/aad82e}{J. Phys. A  {\bf 51}, 39LT01 (2018)}.

\bibitem{Alba2019} V. Alba, B. Bertini and M. Fagotti,
 Entanglement evolution and generalised hydrodynamics: Interacting integrable systems,
\href{https://scipost.org/SciPostPhys.7.1.005}{SciPost Phys. {\bf7}, 005 (2019)}

\bibitem{a-19} V. Alba, {Towards a generalized hydrodynamics description of Renyi entropies in integrable systems},
\href{https://doi.org/https://doi.org/10.1103/PhysRevB.99.045150}{Phys. Rev. B {\bf 99}, 045150 (2019)}.

\bibitem{Calabrese2007} P. Calabrese and J. Cardy,
 Entanglement and correlation functions following a local quench: A conformal field theory approach,
\href{https://iopscience.iop.org/article/10.1088/1742-5468/2007/10/P10004}{J. Stat. Mech. (2007) P10004}

\bibitem{Eisler2008} V. Eisler, D. Karevski, T. Platini and I. Peschel,
 Entanglement evolution after connecting finite to infinite quantum chains,
\href{https://iopscience.iop.org/article/10.1088/1742-5468/2008/01/P01023}{J. Stat. Mech. (2008) P01023}

\bibitem{Eisler2009} V. Eisler, F. Igl\'oi and I. Peschel,
 Entanglement in spin chains with gradients,
\href{https://iopscience.iop.org/article/10.1088/1742-5468/2009/02/P02011}{J. Stat. Mech (2009) P02011}

\bibitem{Igloi2009} F. Igl\'oi, Z. Szatm\'ari and Y. C. Lin,
 Entanglement entropy with localized and extended interface defects,
\href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.80.024405}{Phys. Rev. B {\bf 80}, 024405 (2009)}

\bibitem{Stephan2011} J.-M.  St\'ephan and J. Dubail,
 Local quantum quenches in critical one-dimensional systems: Entanglement, the Loschmidt echo, and light-cone effects,
\href{https://iopscience.iop.org/article/10.1088/1742-5468/2011/08/P08019}{J. Stat. Mech. (2011) P08019}

\bibitem{cc-13} M. Collura and P. Calabrese, {Entanglement evolution across defects in critical anisotropic Heisenberg chains},
\href{http://dx.doi.org/10.1088/1751-8113/46/17/175001}{J. Phys. A {\bf 46}, 175001 (2013)}

\bibitem{Calabrese2016} P. Calabrese and J. Cardy,
 Quantum quenches in 1 + 1 dimensional conformal field theories,
\href{https://iopscience.iop.org/article/10.1088/1742-5468/2016/06/064003}{J. Stat. Mech. (2016) 064003}

\bibitem{Antal1999} T. Antal, Z. R\'acz, A. R\'akos and G. M. Sch\"utz,
 Transport in the XX chain at zero temperature: Emergence of flat magnetization profiles,
\href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.59.4912}{Phys. Rev. E {\bf59}, 4912 (1999)}

\bibitem{Karevski2002} D. Karevski,
 Scaling behaviour of the relaxation in quantum chains,
\href{https://link.springer.com/article/10.1140/epjb/e20020139}{Eur. Phys. J. B {\bf27}, 147 (2002)}

\bibitem{Vicari2012} E. Vicari,
 Quantum dynamics and entanglement in one-dimensional Fermi gases released from a trap.
\href{https://journals.aps.org/pra/abstract/10.1103/PhysRevA.85.062324}{Phys. Rev. A {\bf85}, 062324 (2012)}

\bibitem{Alba2014} V. Alba and F. Heidrich-Meisner,
 Entanglement spreading after a geometric quench in quantum spin chains,
\href{https://journals.aps.org/prb/pdf/10.1103/PhysRevB.90.075144}{Phys. Rev. B {\bf90}, 075144 (2014)}

%%%%%%%%%%%%%%%%%%%%%%%%%%555

\bibitem{chl-08} P. Calabrese, C. Hagendorf, and P. Le Doussal,
{Time evolution of 1D gapless models from a domain-wall initial state: SLE continued?},
\href{http://dx.doi.org/10.1088/1742-5468/2008/07/P07013}{J. Stat. Mech. P07013 (2008)}

\bibitem{Allegra2016} N. Allegra, J. Dubail, J.-M. St\'ephan and J. Viti,
 Inhomogeneous field theory inside the arctic circle,
\href{https://iopscience.iop.org/article/10.1088/1742-5468/2016/05/053108}{J. Stat. Mech. (2016) 053108}

\bibitem{Bertini2018} B. Bertini, L. Piroli and P. Calabrese,
Universal Broadening of the Light Cone in Low-Temperature Transport,
\href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.120.176801}{Phys. Rev. Lett. {\bf120}, 176801 (2018)}

\bibitem{Gruber2019} M. Gruber and V. Eisler,
Magnetization and entanglement after a geometric quench in the XXZ chain,
\href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.99.174403}{Phys. Rev. B {\bf99}, 174403 (2019)}

\bibitem{Lancaster2010} J. Lancaster and A. Mitra,
Quantum quenches in an XXZ spin chain from a spatially inhomogeneous initial state,
\href{https://journals.aps.org/pre/pdf/10.1103/PhysRevE.81.061134}{Phys. Rev. E {\bf 81}, 061134 (2010)}

\bibitem{mpc-10} J. Mossel, G. Palacios, J.-S. Caux, Geometric quenches in quantum integrable systems,
\href{http://dx.doi.org/10.1088/1742-5468/2010/09/L09001}{J. Stat. Mech. (2010) L09001}.

\bibitem{Antal2008} T. Antal, P. L. Krapivsky, and A. R\'akos,
 Logarithmic current fluctuations in nonequilibrium quantum spin chains,
\href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.78.061115}{Phys. Rev. E {\bf78}, 061115 (2008)}

\bibitem{Jin2021} T. Jin, T. Gauti\'e, A. Krajenbrink, P. Ruggiero and T. Yoshimura,
Interplay between transport and quantum coherences in free fermionic systems,
\href{https://arxiv.org/abs/2103.13371}{preprint - arXiv:2103.13371 (2021)}

\bibitem{Cazalilla2004} M. A. Cazalilla,
 Bosonizing one-dimensional cold atomic gases,
\href{https://iopscience.iop.org/article/10.1088/0953-4075/37/7/051}{J. Phys. B {\bf 37}, 1 (2004)}

\bibitem{Giamarchi2007} T. Giamarchi,
\href{https://oxford.universitypressscholarship.com/view/10.1093/acprof:oso/9780198525004.001.0001/acprof-9780198525004}{{\it Quantum Physics in One Dimension}, Oxford Univ. Press (2007)}

\bibitem{next-pub} P. Calabrese, J. Dubail, A. Krajenbrink, and S. Scopa, {\it in preparation}

\bibitem{Jordan1928} P. Jordan and E. Wigner, \"Uber das Paulische \"Aquivalenzverbot. 
\href{https://link.springer.com/article/10.1007/BF01331938}{Z. Phys. {\bf 47}, 631 (1928)}.

\bibitem{Jin2004} B. Q. Jin and V. E. Korepin,
 Quantum spin chain, Toeplitz determinants and the Fisher-Hartwig conjecture,
\href{https://link.springer.com/article/10.1023/B:JOSS.0000037230.37166.42}{J. Stat. Phys. {\bf116}, 79 (2004)}

\bibitem{fg-21} S. Fraenkel and M. Goldstein, Entanglement Measures in a Nonequilibrium Steady State: Exact Results in One Dimension,
 \href{https://arxiv.org/abs/2105.00740 }{preprint - arXiv:2105.00740  (2021)}.

\bibitem{Wendenbaum2013} P. Wendenbaum, M. Collura, and D. Karevski,
 Hydrodynamic description of hard-core bosons on a Galileo ramp,
\href{https://journals.aps.org/pra/abstract/10.1103/PhysRevA.87.023624}{Phys. Rev. A {\bf87}, 023624 (2013)}

\bibitem{Bastianello2020} A. Bastianello, J. Dubail, and J.-M. St\'ephan,
 Entanglement entropies of inhomogeneous Luttinger liquids,
\href{https://doi.org/10.1088/1751-8121/ab7580}{J. Phys. A {\bf 53}, 23 (2020)}

\bibitem{Eisler2013} V. Eisler and Z. R\'acz,
Full counting statistics in a propagating quantum front and random matrix spectra,
\href{https://link.aps.org/doi/10.1103/PhysRevLett.110.060602}{Phys. Rev. Lett. {\bf110}, 060602 (2013)}

\bibitem{Moriya2019} H. Moriya, R. Nagao and T. Sasamoto,
Exact large deviation function of spin current for the one dimensional XX spin chain with domain wall initial condition,
\href{https://iopscience.iop.org/article/10.1088/1742-5468/ab1dd6}{J. Stat. Mech. (2019) 063105}

\bibitem{Bettelheim2011} E. Bettelheim and P. B. Wiegmann,
Universal Fermi distribution of semiclassical nonequilibrium Fermi states,
\href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.84.085102}{Phys. Rev. B {\bf84}, 085102 (2011)}

\bibitem{Bettelheim2012} E. Bettelheim and L. Glazman,
Quantum Ripples Over a Semiclassical Shock,
\href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.109.260602}{Phys. Rev. Lett. {\bf109}, 260602 (2012)}

\bibitem{Wigner1997} E. P. Wigner,
{On the quantum correction for thermodynamic equilibrium},
\href{https://link.springer.com/chapter/10.1007/978-3-642-59033-7_9}{Springer-Verlag Berlin Heidelberg (1997)}

\bibitem{Hinarejos2012} M. Hinarejos, A. P\'erez and M. C. Banuls,
 Wigner function for a particle in an infinite lattice,
\href{https://iopscience.iop.org/article/10.1088/1367-2630/14/10/103009/meta}{New J. Phys. {\bf 14}, 103009 (2012)}

\bibitem{Fagotti2017} M. Fagotti,
Higher-order generalized hydrodynamics in one dimension: The noninteracting test,
\href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.96.220302}{Phys. Rev. B {\bf96}, 220302 (2017)}

\bibitem{Fagotti2020} M. Fagotti,
Locally quasi-stationary states in noninteracting spin chains,
\href{https://scipost.org/10.21468/SciPostPhys.8.3.048}{SciPost Phys. {\bf8}, 048 (2020)}

\bibitem{Moyal1949} J. E. Moyal,
 Quantum mechanics as a statistical theory,
\href{https://www.cambridge.org/core/journals/mathematical-proceedings-of-the-cambridge-philosophical-society/article/abs/quantum-mechanics-as-a-statistical-theory/9D0DC7453AD14DB641CF8D477B3C72A2}{Math. Proc. Cambridge Philos. Soc. {\bf45}, 99 (1949)}

\bibitem{Calabrese2004} P. Calabrese and J. Cardy
Entanglement entropy and quantum field theory,
\href{https://iopscience.iop.org/article/10.1088/1742-5468/2004/06/P06002}{J. Stat. Mech. (2004) P06002}

\bibitem{Cardy2008} J. L. Cardy, O. A. Castro-Alvaredo and B. Doyon,
 Form factors of branch-point twist fields in quantum integrable models and entanglement entropy,
\href{https://link.springer.com/article/10.1007/s10955-007-9422-x}{J. Stat. Phys. {\bf130}, 129 (2008)}

\bibitem{Calabrese2009} P. Calabrese and J. Cardy,
 Entanglement entropy and conformal field theory,
\href{https://iopscience.iop.org/article/10.1088/1751-8113/42/50/504005}{J. Phys. A {\bf 42}, 504005 (2009)}

\bibitem{Calabrese2010} P. Calabrese and F. H.L. Essler,
 Universal corrections to scaling for block entanglement in spin-1/2 XX chains,
\href{https://iopscience.iop.org/article/10.1088/1742-5468/2010/08/P08029}{J. Stat. Mech. (2010) P08029}

\bibitem{cmv-11} P. Calabrese, M. Mintchev, and E. Vicari, {Entanglement Entropy of One-Dimensional Gases}, 
\href{https://doi.org/10.1103/PhysRevLett.107.020601}{Phys. Rev. Lett. {\bf 107}, 020601 (2011)}.

\bibitem{cmv-11b} P. Calabrese, M. Mintchev, and E. Vicari,  {The entanglement entropy of one-dimensional systems in continuous and homogeneous space}, 
\href{http://dx.doi.org/10.1088/1742-5468/2011/09/P09028}{J. Stat. Mech. P09028 (2011)}.

\bibitem{Dubessy2020} R. Dubessy, J. Polo, H. Perrin, A. Minguzzi and M. Olshanii,
Universal shock-wave propagation in one-dimensional Bose fluids, 
\href{https://journals.aps.org/prresearch/abstract/10.1103/PhysRevResearch.3.013098}{Phys. Rev. Res. {\bf3}, 013098 (2021)}

\bibitem{Lieb1961} E. H. Lieb, T. Schultz and D. Mattis, 
Two Soluble Models of an Antiferromagnetic Chain,
\href{https://reader.elsevier.com/reader/sd/pii/0003491661901154?token=0189AFCFF0917F2AD60912AE6437245300497126C5E6E21D5D06CFBFA3D035CC1441288ADCA5FCD47C9D89CEB12BFCD5&originRegion=eu-west-1&originCreation=20210727065759}{Ann. of Phys. {\bf 16}, 407-466 (1961)}

\bibitem{Mukherjee2007} V. Mukherjee, U. Divakaran, A. Dutta and D. Sen,
Quenching dynamics of a quantum XY spin-1/2 chain in a transverse field,
\href{https://journals.aps.org/prb/pdf/10.1103/PhysRevB.76.174303}{Phys. Rev. B {\bf 76}, 174303 (2007)}

\bibitem{Barmettler2010} P. Barmettler, M. Punk, V. Gritsev, E. Demler and E. Altman,
Quantum quenches in the anisotropic spin-1/2 Heisenberg chain: different approaches to many-body dynamics far from equilibrium,
\href{https://iopscience.iop.org/article/10.1088/1367-2630/12/5/055017/pdf}{New J. Phys. {\bf 12}, 055017 (2010)}

\bibitem{Yoshinaga2021} A. Yoshinaga, 
Ballistic propagation in the one-dimensional XY model,
\href{https://iopscience.iop.org/article/10.1088/1742-5468/abcd37}{J. Stat. Mech. (2021) 013103}

\bibitem{p-12} I. Peschel,  Entanglement in solvable many-particle models,
 \href{http://dx.doi.org/10.1007/s13538-012-0074-1}{Braz. J. Phys. {\bf 42}, 267 (2012)}.

\bibitem{Peschel1999a} I. Peschel, M. Kaulke and \"O. Legeza,
 Density-matrix spectra for integrable models,
\href{https://doi.org/10.1002/(SICI)1521-3889(199902)8:2<153::AID-ANDP153>3.0.CO;2-N}{Ann. Phys. {\bf8}, 153 (1999)}

\bibitem{Chung2001} M. C. Chung and I. Peschel,
 Density-matrix spectra of solvable fermionic systems,
\href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.64.064412}{Phys. Rev. B {\bf64}, 064412 (2001)}

\bibitem{Peschel2003} I. Peschel,
 Calculation of reduced density matrices from correlation functions,
\href{https://iopscience.iop.org/article/10.1088/0305-4470/36/14/101}{J. Phys. A {\bf36}, L205 (2003)}

\bibitem{Peschel2004} I. Peschel,
 On the reduced density matrix for a chain of free electrons,
\href{https://iopscience.iop.org/article/10.1088/1742-5468/2004/06/P06004}{J. Stat. Mech. (2004) P06004}

\bibitem{Peschel2009} I. Peschel and V. Eisler,
 Reduced density matrices and entanglement entropy in free lattice models,
\href{https://iopscience.iop.org/article/10.1088/1751-8113/42/50/504003}{J. Phys. A {\bf42}, 504003 (2009)}


\end{thebibliography}

%%%%% CLEAR DOUBLE PAGE!
\newpage{\pagestyle{empty}\cleardoublepage}
